What a Whole Slide Image Can Tell? Subtype-guided Masked Transformer for Pathological Image Captioning

Pathological captioning of Whole Slide Images (WSIs), though is essential in computer-aided pathological diagnosis, has rarely been studied due to the limitations in datasets and model training efficacy. In this paper, we propose a new paradigm Subtype-guided Masked Transformer (SGMT) for pathological captioning based on Transformers, which treats a WSI as a sequence of sparse patches and generates an overall caption sentence from the sequence. An accompanying subtype prediction is introduced into SGMT to guide the training process and enhance the captioning accuracy. We also present an Asymmetric Masked Mechansim approach to tackle the large size constraint of pathological image captioning, where the numbers of sequencing patches in SGMT are sampled differently in the training and inferring phases, respectively. Experiments on the PatchGastricADC22 dataset demonstrate that our approach effectively adapts to the task with a transformer-based model and achieves superior performance than traditional RNN-based methods. Our codes are to be made available for further research and development.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> tables/aug.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}

\begin{table}[t]
    \caption{Performance comparison on Camelyon val set and test set.}
    \centering
    \resizebox{0.99\columnwidth}{!}{
    \tablestyle{1pt}{1.0}
    \begin{tabular}{@{}llcc@{}}
        \toprule
        Algorithm & Backbone & Val Acc(Center 4)& Test Acc (Center 5) \\ \midrule
        CORAL \cite{koh2021wilds}             & DenseNet121   & 86.2 & 59.5 \\
        IRM \cite{koh2021wilds}              & DenseNet121   & 86.2 & 64.2 \\
        %Group DRO \cite{koh2021wilds}        & DenseNet121   & 85.5 & 68.4 \\
        CGD \cite{piratla2021focus}        & DenseNet121   & 86.8 & 69.4 \\
        Fish \cite{shi2021gradient}             & DenseNet121   & 83.9 & 74.1 \\
        LISA \cite{yao2022improving}             & DenseNet121   & 81.8 & 77.1 \\
        %ERM (grid search) \cite{koh2021wilds}   & DenseNet121   & 84.9 & 70.3 \\
        %ERM (rand search) \cite{sagawa2021extending} & DenseNet121   & 85.8 & 70.8 \\
        ERM w/ data aug \cite{sagawa2021extending}   & DenseNet121  & 90.6 & 82.0 \\
        ERM w/ targeted aug \cite{gao2022out}   & DenseNet121  & 92.7 & 92.1 \\
        ERM w/ H\&E jitter \cite{8327641} & SE-ResNeXt101  & 88.0 & 91.6 \\
        \midrule
        Normal Training                & SE-ResNeXt101 & 75.3     & 57.2     \\
        Augmix \cite{hendrycks2019augmix}            & SE-ResNeXt101 & 86.6     & 76.9     \\
        \textbf{Ours (+OmniCE)} & \textbf{SE-ResNeXt101} & \textbf{94.9}     & \textbf{92.2}     \\ 
        \bottomrule
        \end{tabular}
    }
    \label{table:aug}
\end{table}


==> tables/crc.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}

\begin{table*}[!t]
    %\caption{Average ACC of Models}
    \caption{\label{tab1}CRC dataset mBCE  }
    \centering
    \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllllllllllllllllllll@{}}
\toprule
architecture &
  error &
  mBCE &
  HE shallow &
  HE deep &
  H shallow &
  H deep &
  E shallow &
  E deep &
  HE region &
  H region &
  E region &
  uneven &
  defocus &
  cold &
  warm &
  overexposure &
  underexposure &
  dent &
  bubble &
  crack &
  knife \\ \midrule
Alexnet &
  8.41 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 &
  100.00 \\
VGG16 &
  3.90 &
  61.74 &
  48.03 &
  54.57 &
  81.49 &
  64.91 &
  47.42 &
  67.65 &
  37.41 &
  38.46 &
  43.23 &
  39.41 &
  100.88 &
  43.57 &
  77.80 &
  168.87 &
  78.78 &
  42.83 &
  66.16 &
  40.19 &
  31.49 \\
ResNet18 &
  6.41 &
  97.96 &
  75.41 &
  140.69 &
  97.54 &
  141.00 &
  66.70 &
  151.45 &
  58.00 &
  58.72 &
  56.17 &
  104.97 &
  150.84 &
  102.95 &
  93.61 &
  251.85 &
  79.44 &
  65.09 &
  78.52 &
  38.51 &
  49.74 \\
ResNet50 &
  6.69 &
  98.38 &
  71.10 &
  104.47 &
  108.89 &
  151.92 &
  54.83 &
  122.85 &
  67.03 &
  73.38 &
  62.03 &
  86.25 &
  128.29 &
  113.38 &
  93.23 &
  226.88 &
  154.57 &
  75.21 &
  71.19 &
  48.95 &
  54.77 \\
ResNet101 &
  5.85 &
  112.17 &
  111.58 &
  114.83 &
  128.43 &
  154.28 &
  49.68 &
  110.30 &
  94.38 &
  113.81 &
  60.18 &
  112.67 &
  206.67 &
  152.99 &
  95.53 &
  280.10 &
  124.78 &
  61.70 &
  64.32 &
  50.02 &
  44.88 \\
DenseNet121 &
  4.96 &
  94.25 &
  67.11 &
  113.42 &
  87.98 &
  102.71 &
  44.34 &
  126.53 &
  53.33 &
  68.37 &
  50.06 &
  91.03 &
  164.18 &
  191.79 &
  82.57 &
  263.51 &
  94.48 &
  53.35 &
  63.41 &
  32.66 &
  39.92 \\ \bottomrule
    \end{tabular}%
    }
    \end{table*}

==> tables/pcam2.tex <==
\begin{table*}[t]
    \centering
    \caption{Error rate results ($\downarrow$) of the patch level OmniCE corruption benchmark datasets. 
    The best and worst results among models are marked by \textbf{value} and \underline{value} for every row, \textcolor{blue}{value} and \textcolor{red}{value} for every column.}
    %We train on clean images and test on this benchmark. 
    %For every row, the best and worst results among models are marked by \textbf{value} and \underline{value}. For every column, the best and worst results among corruptions are marked by \textcolor{blue}{value} and \textcolor{red}{value}.}
    \resizebox{2\columnwidth}{!}{
    \tablestyle{1pt}{1}
    \begin{tabular}{l|rr|rr|rr|rr|rr|rr||rr|rr|rr|rr|rr|rr}
    \toprule\toprule
     \multicolumn{1}{c}{}&\multicolumn{12}{c||}{PatchCamelyon} &\multicolumn{12}{c}{CRC-HE}\\
    \toprule\toprule
    
         \multirow{2}{*}{OmniCE}& \multicolumn{2}{c|}{AlexNet}& \multicolumn{2}{c|}{VGG16} & \multicolumn{2}{c|}{ResNet18} & \multicolumn{2}{c|}{ResNet50} & \multicolumn{2}{c|}{ResNet101} & \multicolumn{2}{c||}{DenseNet121}& \multicolumn{2}{c|}{AlexNet} & \multicolumn{2}{c|}{VGG16} & \multicolumn{2}{c|}{ResNet18} & \multicolumn{2}{c|}{ResNet50} & \multicolumn{2}{c|}{ResNet101} & \multicolumn{2}{c}{DenseNet121} \\ %\midrule
       &mCE&rCE&mCE&rCE&mCE&rCE&mCE&rCE&mCE&rCE&mCE&rCE&mCE&rCE&mCE&rCE&mCE&rCE&mCE&rCE&mCE&rCE&mCE&rCE\\
        \midrule\midrule
        
        Under-stained  H\&E & \underline{100.0} & \textbf{2.3} & 55.8 & 3.9 & \textbf{45.3} & 3.1 & 55.6& 3.7 & 55.1 & 3.7 & 62.6 & \underline{5.1} & 100.0 & 4.6& \textbf{48.0} & 4.8 & 75.4 & 4.6 & 71.1& \textbf{4.1} &\underline{111.6}  &\underline{7.4}  & 67.1&5.3 \\ 
        Over-stained  H\&E& \underline{100.0} & 2.0  & \textbf{31.3} & \textbf{1.9} & 37.6 & 2.3 & 55.6& \underline{3.3} & 44.1 & 2.6 & 46.1 & \underline{3.3}& 100.0 & \textbf{3.3}& \textbf{54.6} & 3.9 & \underline{140.7}& 6.1 & 104.5 &4.4 & 114.8 &5.5  & 113.4 &\underline{6.4}  \\  
         Under-stained  H& \underline{100.0} & \textbf{2.3}   & 59.7 & 4.2 & \textbf{52.9} & 3.7 & 57.6& 3.8 & 53.4 & 3.6 & 53.6&\underline{4.4} & 100.0 & \textbf{4.6}& \textbf{81.5} & 8.1 & 97.5 & 5.9 & 108.9& 6.3 &\underline{128.4}  &\underline{8.5}  &88.0 &6.8 \\ 
         Over-stained  H& \underline{100.0} & 1.9   & 32.0 & 1.8 & 36.6 & 2.1 & 44.1& \underline{2.4} & 28.9 & \textbf{1.6} & \textbf{27.3} & 1.8& 100.0 & \textbf{2.7}& \textbf{64.9} & 3.8 & 141.0& 5.1 & 151.9 &5.2 & \underline{154.3} &\underline{6.1}  & 102.7 &4.8  \\  
         Under-stained  E& \underline{100.0} & \textbf{1.5}   & 42.2 & 1.9 & \textbf{34.2} & 1.6 & 39.6& 1.7 & 35.0 & \textbf{1.5} & 36.8&\underline{2.0}& \underline{100.0} & \underline{2.4}& 47.4 & \underline{2.4} &66.7 &2.1  & 54.8 &\textbf{1.6} &49.7  &1.7  & \textbf{44.3} &1.8  \\  
         Over-stained  E& \underline{100.0} & \textbf{2.3}   & \textbf{43.4} & 3.0 & 61.3 & 4.2 & 78.6& 5.2 & 51.3 & 3.4 & 66.4 & \underline{5.4}& 100.0 & \textbf{3.2}& \textbf{67.6} & 4.7 &\underline{151.5} &6.4  &122.8  &5.0 &  110.3&5.1  & 126.5 &\underline{6.9}  \\  
         Residual Wax& \underline{100.0} & \textbf{1.7}   & 37.4 & 1.9 & \textbf{33.1} & \textbf{1.7} & 37.2& 1.8 & 36.2 & 1.8 & 40.6 & \underline{2.4}& \underline{100.0} & 1.6 & \textbf{37.4} & 1.3 &58.0 &\textbf{1.2}  &67.0  &1.4 & 94.4 &\underline{2.2}  &53.3  & 1.5 \\ 
         Residual Xylene& \underline{100.0} & 1.7   & 34.2 & 1.8 & \textbf{30.7} & \textbf{1.6} & 35.6& 1.7 & 35.9 & 1.8 & 31.1 & \underline{1.9}& 100.0 & 1.5 & \textbf{38.5} & 1.2 &58.7 &\textbf{1.1}  &73.4  &1.4 & \underline{113.8} &\underline{2.4}  &68.4  &1.7  \\  
         Residual Alkali& \underline{100.0} & \textbf{1.3}   & 36.3 & 1.4 & 32.8 & \textbf{1.3} & 37.8& 1.4 & 36.1 & \textbf{1.3} & \textbf{32.3} & \underline{1.5}& \underline{100.0} & \underline{1.3} & \textbf{43.2} & 1.2 & 56.2&\textbf{\textcolor{blue}{1.0}}  & 62.0 &\textbf{\textcolor{blue}{1.0}} & 60.2 &1.1  &50.1  &1.1  \\ 
         Thick and Thin& \underline{100.0} & \textbf{1.8}   & 35.2 & 1.9 & \textbf{33.9} & \textbf{1.8} & 42.3& 2.1 & 39.5 & 2.0 & 42.8 & \underline{2.7}& 100.0 & 2.4 & \textbf{39.4} & \textbf{2.0} &105.0 &3.3  &86.3  &2.6 &\underline{112.7}  &\underline{3.9}  & 91.0 &3.7  \\  
        \midrule
        Stain Deposit& \underline{100.0} & \underline{1.4}   & \textcolor{blue}{25.6} & \textcolor{blue}{1.1} & \textcolor{blue}{23.5} & \textbf{\textcolor{blue}{1.0}} & \textcolor{blue}{26.9}& \textcolor{blue}{1.1} & \textcolor{blue}{26.1} & 1.1 & \textbf{\textcolor{blue}{22.5}} & \textcolor{blue}{1.1} & \underline{100.0} & \underline{1.2} & \textbf{42.8} & 1.1 & 65.1 & \textbf{\textcolor{blue}{1.0}} &75.2 &\underline{1.2}  & 61.7 &1.1  & 53.3&1.1 \\ 
         Bubble& \underline{100.0} & \textbf{\textcolor{blue}{1.1}}   & 42.9 & 1.4 & 46.5 & 1.5 & 53.7& \underline{1.6} & 51.0 & \underline{1.6} & \textbf{37.4} & 1.4& \underline{100.0} & \textcolor{blue}{1.1} & 66.2 & \underline{1.6} &78.5 &1.2  &71.2  & \textbf{\textcolor{blue}{1.0}}& 64.3 &\textbf{\textcolor{blue}{1.0}}  & \textbf{63.4} &1.2  \\  
        
         Knife Line& \underline{100.0} & \underline{\textcolor{blue}{1.1}}   & 35.5 & \underline{\textcolor{blue}{1.1}} & 31.8 & \textbf{\textcolor{blue}{1.0}} & 34.6& \underline{\textcolor{blue}{1.1}} & 33.6 & \textbf{\textcolor{blue}{1.0}} & \textbf{29.1} & \underline{\textcolor{blue}{1.1}}& \underline{100.0} & \underline{1.5} & \textbf{\textcolor{blue}{31.5}} & \textbf{\textcolor{blue}{1.0}} & 49.7&\textbf{\textcolor{blue}{1.0}}  & 54.8 &1.1 & \textcolor{blue}{44.9} &\textbf{\textcolor{blue}{1.0}}  & 39.9 &\textbf{\textcolor{blue}{1.0}}  \\  
        %\midrule
        Crack& \underline{100.0} & \textbf{1.2}  & 53.6 & 2.0 & 56.3 & 2.1 & 54.5& 1.9 & 50.7 & 1.8 & \textbf{49.3} & \underline{2.2} & \underline{100.0} & \underline{2.5} & 40.2 & 2.2 & \textcolor{blue}{38.5} &\textbf{1.3}  & \textcolor{blue}{49.0}& 1.5 & 50.0 &1.8  &\textbf{\textcolor{blue}{32.7}} &1.4 \\ 
        \midrule\midrule
        
         Cold Color& 100.0 & \textbf{2.0}   & 88.6 & 5.3 & \textbf{71.3} & 4.3 & 84.6& 4.8 & \underline{106.3} & \underline{6.1} & 79.0 & 5.6& 100.0 & 3.2 & \textbf{43.6} & \textbf{3.1} & 102.9&4.4  & 113.4 &4.6 & 153.0  & 7.1 & \underline{191.8} &\underline{10.6}  \\  
         Warm Color& \underline{100.0} & \textbf{\textcolor{red}{3.0}}   & \textbf{83.1} & 7.6 & 89.9 & \textcolor{red}{8.2} & 91.0& \textcolor{red}{7.9} & 85.5 & 7.5 & 84.5 & \underline{\textcolor{red}{9.1}} & \underline{100.0} & \textbf{\textcolor{red}{7.5}} & \textbf{77.8} & \underline{\textcolor{red}{12.6}} & 93.6 &9.2  & 93.2& \textcolor{red}{8.8} & 95.5 & 10.3 & 82.6 &10.5 \\ 
         Overexposure& \textbf{100.0} & \textbf{2.0}   & \textcolor{red}{127.3} & \textcolor{red}{7.7} & 112.7 & 6.8 & \textcolor{red}{125.9}& 7.2 & \underline{\textcolor{red}{142.2}} & \textcolor{red}{8.2} & \textcolor{red}{121.1} & \underline{8.6} & \textbf{100.0} & \textbf{3.0} & \textcolor{red}{168.9} & 11.0 &\textcolor{red}{251.9}  &\textcolor{red}{9.9}  &\textcolor{red}{226.9} &8.6  & \underline{\textcolor{red}{280.1}} &\textcolor{red}{12.1}  & \textcolor{red}{263.5}&\underline{\textcolor{red}{13.5}} \\ 
         Underexposure& 100.0 & \textbf{1.7}  & \textbf{90.9} & 4.8 & \textcolor{red}{117.3} & 6.2 & 114.3& 5.7 & \underline{136.1} & \underline{6.9} & 107.3 & 6.6 & 100.0 & \textbf{2.0} & \textbf{78.8} & 3.4 & 79.4 &2.1  & \underline{154.6}& \underline{3.9} & 124.8 &3.6  &94.5 &3.2 \\
        
        
        Defocus& 100.0 & \textbf{2.4}   & 97.0 & 7.0 & 97.4 & 7.0 & \underline{100.6}& 6.9 & \textbf{81.7} & 5.7 & 90.4 & \underline{7.7}& \textbf{100.0} & \textbf{2.7} & 100.9 & 5.9 &150.8 &5.4  & 128.3 &4.4 & \underline{206.7} &\underline{8.1}  &164.2  & 7.6 \\  
         \midrule\midrule
        Average& \underline{100.0} & \textbf{1.8}   & 55.4 & 3.3 & \textbf{55.0} & 3.2 & 61.6& 3.4 & 59.4 & 3.3  & 55.8 & \underline{3.9}& 100.0 & \textbf{2.8} & \textbf{61.7} & 4.0 & 98.0&3.8 & 98.4& 3.6 & \underline{112.2} & \underline{4.7} & 94.3 & \underline{4.7}\\ 
        %\midrule
        Original Error & \multicolumn{2}{c|}{\underline{12.9}} & \multicolumn{2}{c|}{4.2} & \multicolumn{2}{c|}{4.2} & \multicolumn{2}{c|}{4.5}& \multicolumn{2}{c|}{4.4}&  \multicolumn{2}{c||}{\textbf{3.6}} &\multicolumn{2}{c|}{\underline{8.4}}& \multicolumn{2}{c|}{\textbf{3.9}} & \multicolumn{2}{c|}{6.4} & \multicolumn{2}{c|}{6.7}& \multicolumn{2}{c|}{5.9}& \multicolumn{2}{c}{5.0} \\ 
        
        \bottomrule\bottomrule
    \end{tabular}
    }
    \label{table:pcam2}
    %\vspace{-3mm}
\end{table*}

==> tables/seg.tex <==
\begin{table}[t]
    \centering
    \tiny
    \caption{Dice score results ($\uparrow$) of the slide level OmniCE corruption benchmark dataset. 
    %We train on clean images and test on this benchmark. For every row, the best and worst results among models are marked by \textbf{value} and \underline{value}. For every column, the best and worst results among corruptions are marked by \textcolor{blue}{value} and \textcolor{red}{value}. 
    The best and worst results are marked in the same way as in Table \ref{table:pcam2}.}
    \resizebox{0.99\columnwidth}{!}{
    \tablestyle{15pt}{1.0}
    \begin{tabular}{@{}l|cccc}
    \toprule\toprule
        OmniCE & UNet & GCN & DCAN & Dense-UNet \\ %
        \midrule\midrule
        
        Under-stained H\&E & \textbf{0.6138} & 0.5668 & \underline{0.3968} & 0.5724  \\ 
         Over-stained  H\&E & \textbf{0.7438} & 0.7137 & \underline{0.6088} & 0.7194 \\ 
         Under-stained H & \textcolor{red}{0.3450} & 0.4454 & \underline{0.2415} & \textbf{0.4496}  \\ 
         Over-stained  H & \textbf{0.7435} & 0.7291 & \underline{0.6378} & 0.7416  \\ 
         Under-stained E & \textbf{0.7620} & 0.7283 & \underline{0.6183} & 0.7349  \\ 
         Over-stained  E & 0.6312 & 0.6649 & \underline{0.4729} & \textbf{0.6768}  \\ 
         Residual Wax & \textbf{0.7690} & 0.7243 & \underline{0.6560} & 0.6950  \\
         Residual Xylene & \textbf{0.7620} & 0.7184 & \underline{0.6482} & 0.6882 \\ 
         Residual Alkali & \textbf{0.7736} & 0.7332 & \underline{0.6635} & 0.7404 \\
         Thick and Thin & \textbf{0.7535} & 0.7030 & \underline{0.6281} & 0.7091 \\ 
         \midrule
         Stain Deposit & \textbf{0.7749} & \underline{0.7408} & \textbf{0.7749} & 0.7504  \\ 
         Bubble & \textcolor{blue}{0.7750} & \underline{\textcolor{blue}{0.7419}} & \textbf{\textcolor{blue}{0.7751}} & \textcolor{blue}{0.7539} \\ 
        
         Knife Line & 0.6912 & \textbf{0.7023} & \underline{0.6721} & 0.7015 \\ 
         %\midrule
         Crack & \textbf{0.7651} & 0.7174 & \underline{0.6690} & 0.7110  \\ 
         Fold & \textbf{0.7253} & 0.6626 & \underline{0.6254} & 0.6499\\ 
         Venetian & \textbf{0.6813} & 0.6340& \underline{0.6183} & 0.6512\\ 
         \midrule\midrule
         
         
         Cold Color & \textbf{0.7727} & 0.6234 & \underline{0.2383} & 0.6337 \\ 
         Warm Color & \textbf{0.6745} & 0.4629 & \underline{0.1168} & \textcolor{red}{0.3573}\\ 
         Overexposure & \textbf{0.3937} & \textcolor{red}{0.1673}& \underline{\textcolor{red}{0.1100}}& 0.3614 \\ 
         Underexposure & \textbf{0.6622} &0.6424 & \underline{0.3888} & 0.6098 \\
         %\midrule
        Defocus & \textbf{0.7181}  & 0.6231  &  \underline{0.612} & 0.6731 \\ 
        \midrule\midrule
        Average & \textbf{0.6920} & 0.6402 &  \underline{0.5320}& 0.6467 \\ 
        %\midrule
       Original & 0.7812 & \underline{0.7457} & \textbf{0.7831} & 0.7583 \\
        
        \bottomrule\bottomrule
    \end{tabular}
    }
    \label{table:seg}
\end{table}
